Soteria: A Provably Compliant User Right Manager Using a Novel Two-Layer Blockchain Technology

Soteria is a user right management system designed to safeguard user-data privacy in a transparent and provable manner in compliance to regulations such as GDPR and CCPA. Soteria represents user data rights as formal executable sharing agreements, which can automatically be translated into a human readable form and enforced as data are queried. To support revocation and to prove compliance, an indelible, audited trail of the hash of data access and sharing agreements are stored on a two-layer distributed ledger. The main chain ensures partition tolerance and availability (PA) properties while side chains ensure consistency and availability (CA), thus providing the three properties of the CAP (consistency, availability, and partition tolerance) theorem. Besides depicting the two-layer architecture of Soteria, this paper evaluates representative consensus protocols and reports performance statistics.

==> APIs-Old-With-Figures.tex <==
\section{Appendix --- API Specifications}
\label{sec-specs}

Figures \ref{fig:system_workflow_registration} to \ref{fig:system_workflow_invocation} illustrate the workflows of {\em user registration} (UR), {\em data entry creation \& deletion} (DEC \& DED), 
{\em EAS deployment} (EASD), and {\em EAS invocation \& revocation}
(EASI \& EASR), respectively.  For each transaction, we first 
depict its API signature (detailed specifications are documented in
the Appendix) and then explain its workflow.  In addition to these six transactions, which 
create indelible records on DTL, DataXchange also provides 
{\em data query service} (DQS) for users to search for matching data. DQS
is not a traction because we do not record search activities on DTL.


\subsection {User Registration (UR)}
{\bf API}: {\em POST /user/register/ : register a user (provider or consumer)}

\noindent Figure~\ref{fig:system_workflow_registration} shows the UR workflow of three steps.
\begin{enumerate}
\item Each user must register an account with DataXchange via a web application.
An ER request requires an user type (provi-\\der or consumer), an ID and a password.
\item Once a user has submitted his/her registration, a new account is created, consisting of an user-specified ID and a generated DTL keystore file, including a DTL account address and an encrypted private key, for user identification on the ledger. Then, the web application submits a UR request with the user type, the user-specified ID and the DTL account address to DDS.
\item DDS receives the UR request and sends an UR-TX with the user-specified ID and the DTL account address to the data directory on DTL. Meanwhile, this UR information is stored in DDS' storage.
\end{enumerate}

\begin{figure*}[h]
\begin{center}
\includegraphics[width=14cm]{Images/DataXchangeWorkFlow-registration-Alison.png}
\end{center}
\caption{The workflow of user registration}
\label{fig:system_workflow_registration}
\end{figure*}


\subsection {Data Entry Creation and Deletion (DEC \& DED)}

{\bf API}: {\em POST /entry/create/ : create a new data entry by a provider} \\
{\bf API}: {\em POST /entry/delete/ : delete a new data entry by a provider}

\noindent Figure~\ref{fig:system_workflow_creation} shows the DEC and DED workflows.

\begin{enumerate}
\item A data provider logs onto DDS and fills out a DEC form, including data provider address, data certificate, data owner code, data entry title, data description, data access path, expiration date, and/or data offer price if applicable. Note that the data provider address is derived from the data provider ID; also, the data entry creation date and the data offer status are set by DDS. Note that the data certificate is generated by the provided tool of certificate generator.
\item The web application creates a transaction with the inserted form field values as the transaction data, signs this transaction with the  provider's private key (signature), and submits a DEC request to DDS.
\item Once the DEC request is received, DDS checks whether the data provider's account is registered.
\item DDS sends a DEC-TX to the {\em data directory} on the ledger.
\item After receiving the DEC-TX, the DED-TX is thus stored as an activity event for {\em data activity logging}.
\item This DEC information is synchronized to the {\em directory storage} and {\em audit log storage}.
\item Furthermore, the data provider can send a DED request via the web application to DDS for entry deletion when needed. DDS subsequently sends a DED-TX to the {\em data directory} on the ledger. A DED transaction (DED-TX) consists of the same field values as DEC-TX, except that the data offer status is set to {\em false} to make this data entry unviewable by DDS. After receiving the DED-TX, the DED-TX is stored as an activity event for {\em data activity logging}. Finally, this DED information is synchronized to the {\em directory storage} and {\em audit log storage}.
\end{enumerate}

\begin{figure*}[h]
\begin{center}
\includegraphics[width=14cm]{Images/DataXchangeWorkFlow-creation-Alison.png}
\end{center}
\caption{The workflow of data entry creation}
\label{fig:system_workflow_creation}
\end{figure*}


\subsection {EAS Deployment (EASD)}

{\bf API}: {\em POST /entry/deploy/ : deploy a new EAS for a provider and a consumer}

\noindent Figure~\ref{fig:system_workflow_deployment} shows the workflow of EASD.

\begin{enumerate}
 \item A data consumer browses the results of a search on DDS, chooses desired data items, and sends an agreement via the web application. The agreement is signed with the data consumer's private key (signature).

\item The web application submits the request with the data consumer ID and the signed data consumer's agreement to DDS. At this stage, the agreement is considered a bid with terms (e.g., expiration date and price).
% content of the agreement needs to be defined

\item Once the data consumer's agreement request is received, DDS checks whether the data consumer's account is valid, and stores the signature in the {\em directory storage}.

\item The data provider checks its data items prescribed by the data consumer via the web interface. If the data provider  decides to reply an agreement, either accepting it or proposing new terms, a replied agreement is sent via the web application. The agreement is signed with the data provider's private key (signature).

\item The web application submits the request with the data provider ID and the signed data provider's agreement to DDS. % content of the agreement needs to be defined

\item Once the data provider's agreement is received, DDS checks whether the data provider's account is valid, and stores the signature in the {\em directory storage}.

\item After the bi-directional agreements are both received, DDS confirms whether both parties\footnote{Note that the data consumer address and data provider address are derived from the IDs stored in the agreements, and the data consumer's signature and data provider's signature are retrieved from the {\em directory storage}. Besides, the deployment date and the validity status are set by DDS.} can enter a contract.
If so, DDS signs and sends an EASD-TX to the {\em data directory} on the ledger.  If not, DDS returns to the
data consumer with a reason code.  The consumer can consider to rebid, or terminate.

\item The {\em data directory} creates a new EAS on the ledger. In other words, the EAS for both data provider and data consumer is established and triggered\footnote{EAS stores the data provider address, data consumer address, data certificate, data owner code (de-identified), data entry title, data description, data access path, agreement terms, data provider's agreement, data consumer's agreement, EAS deployment date and EAS validity status (set to {\em true}). Note that the data provider address, data certificate, data owner code (de-identified), data entry title, data description, data access path and data conditions are retrieved from the corresponding data entry.}.

\item After receiving the EASD-TX, the EASD-TX is stored as an activity event for {\em data activity logging}.

\item This EASD information is synchronized to the {\em directory storage} and {\em audit log storage}.
\end{enumerate}

\begin{figure*}[ht]
\begin{center}
\includegraphics[width=14cm]{Images/DataXchangeWorkFlow-deployment-Alison.png}
\end{center}
\caption{The workflow of EAS deployment}
\label{fig:system_workflow_deployment}
\end{figure*}

\subsection {EAS Invocation and Revocation (EASI \& EASR)}


{\bf API}: {\em POST /eas/invoke/ : log an access result when an EAS is invoked} \\
{\bf API}: {\em POST /eas/revoke/ : revoke an EAS by a user (provider or consumer)}

\noindent Figure~\ref{fig:system_workflow_invocation} depicts the workflows of EASI and EASR.

\begin{enumerate}
\item Before an EAS deployment, the provider inserted for each data item a data registry (with data certificate and data access script) into the registry storage of the provider's data server.
\item After EASD, the consumer is noticed that an EAS has been created. The consumer can now send a download access request for this data item via the web application.
\item The web application submits the download access request with the data consumer's signature to the provider's data server via the data access script (e.g., the provider server's REST API).
\item After receiving the request, the provider server retrieves the corresponding EAS content on the ledger to check the offer conditions, the validity status and the data consumer's signature. If the access time has expired or the validity status is {\em false}, the data download access is denied (denoted as ``validation failed''). 
\item The provider server sends a validation passed/failed result signed with the data provider's private key (signature) to DDS.
\item Once the provider server's result is received, DDS checks whether the data provider's account is registered, and then sends an EASI-TX with the validation result to the {\em data directory} on the ledger.
\item After receiving the EASI-TX, the EASI-TX is stored as an activity event for {\em data activity logging}.
\item On step (5), if the validation passes, the provider server sends a request to the data server (both are managed data provider service) to apply the real download link for the data consumer with an expiration time stamp. 
%The purpose of this design is to avoid real data file path exposure (on data entry) problem and download link spreading problem for security. In addition, this design also meet the timely access requirement for data expiration date.
\item The data provider thus transfers the data to the data consumer via the real download link (or access script).
\item After the data is downloaded by the data consumer, the consumer verify data authenticity via the certificate server.
\item This EASI information is synchronized to the {\em directory storage} and {\em audit log storage}.
\item Furthermore, the data provider or data consumer can send an EASR request via the web application to DDS for revocation (disable the data access) when desired. DDS subsequently sends an EASR-TX to the {\em data directory} on the ledger. 
%To send an EASR-TX, the form fields of data provider ID, data consumer ID and data certificate are required. Note that data provider address and data consumer address are derived from the IDs; also, the form field of validity status is set to {\em false} by DDS. An EASR-TX is signed with the data provider's private key (signature) or the data consumer's private key (signature). 
After receiving the EASR-TX, the EASR-TX is stored as an activity event for {\em data activity logging} with
validity status set to {\em false}. 
Finally, this EASR information is synchronized to the {\em directory storage} and {\em audit log storage}. 
Note that the data consumer cannot send the EASR request after the data has been downloaded by that consumer.
\end{enumerate}

\begin{figure*}[ht]
\begin{center}
\includegraphics[width=14cm]{Images/DataXchangeWorkFlow-invocation-Alison.png}
\end{center}
\caption{The workflow of EAS invocation and revocation}
\label{fig:system_workflow_invocation}
\end{figure*}


\subsection {Data Query Service (DQS)}
{\bf API}:{\em GET /entry/search/ : retrieve data entries with a search query}

\noindent Figure~\ref{fig:system_workflow_search} depicts the workflow of DQS.

\begin{enumerate}
\item Any registered user can log onto DDS to issue a query with desired criteria (e.g., disease name, gender,
and age) via the web application to find matching data entries.
\item DDS retrieves from its {\em directory storage} based on the query criteria.
\item DDS returns matching data entries to the querier.
\end{enumerate}

\begin{figure*}[ht]
\begin{center}
\includegraphics[width=14cm]{Images/DataXchangeWorkFlow-search-Alison.png}
\end{center}
\caption{The workflow of data query service}
\label{fig:system_workflow_search}
\end{figure*}

==> APIs.tex <==
\section*{Appendix --- Transaction API Specifications}
\label{sec-specs}

\begin{figure*}[h!]
\begin{center}
\includegraphics[width=13cm]{Images/Soteria-arch.png}
\end{center}
\caption{The Workflow of User Registration.}
\label{fig:system_workflow_search}
\end{figure*}



%Figures \ref{fig:system_workflow_registration} to \ref{fig:system_workflow_invocation} illustrate the workflows of 
This appendix specifies the APIs and workflow of \Soteria's six transactions:
{\em user registration} (UR), {\em data entry creation \& deletion} (DEC \& DED), 
{\em ESA deployment} (ESAD), and {\em ESA invocation \& revocation}
(ESAI \& ESAR), respectively.  
%In addition to these six transactions, which create indelible records on DTL, \Soteria also provides {\em data query service} (DQS) for users to search for matching data. DQS is not a traction because we do not record search activities on DTL.

\subsection*{User Registration (UR)}
\noindent
{\bf API}: {\em POST /user/register/ : register a user}

%\noindent Figure~\ref{fig:system_workflow_registration} shows the UR workflow of three steps.
\begin{enumerate}
\item Each user must register an account with \Soteria via a web application.
An ER request requires an user type (provi-\\der or consumer), an ID and a password.
\item Once a user has submitted his/her registration, a new account is created, consisting of an user-specified ID and a generated DTL keystore file, including a DTL account address and an encrypted private key, for user identification on the ledger. Then, the web application submits a UR request with the user type, the user-specified ID and the DTL account address to DDS.
\item DDS receives the UR request and sends an UR-TX with the user-specified ID and the DTL account address to the data directory on DTL. Meanwhile, this UR information is stored in DDS' storage.
\end{enumerate}


%\begin{figure*}[h]
%\begin{center}
%\includegraphics[width=14cm]{Images/DataXchangeWorkFlow-creation-Alison.png}
%\end{center}
%\caption{The workflow of data entry creation}
%\label{fig:system_workflow_creation}
%\end{figure*}


\subsection*{ESAD: EAS Deployment}
\noindent
{\bf API}: {\em POST /entry/deploy/ : deploy a new ESA for a provider and a consumer}

%\noindent Figure~\ref{fig:system_workflow_deployment} shows the workflow of EASD.

\begin{enumerate}
 \item A data consumer browses the results of a search on URM, chooses desired data items, and sends an agreement via the web application. The agreement is signed with the data consumer's private key (signature).

\item The web application submits the request with the data consumer ID and the signed data consumer's agreement to URM. At this stage, the agreement is considered a bid with terms (e.g., expiration date and price).
% content of the agreement needs to be defined

\item Once the data consumer's agreement request is received, DDS checks whether the data consumer's account is valid, and stores the signature in the {\em directory storage}.

\item The data provider checks its data items prescribed by the data consumer via the web interface. If the data provider  decides to reply an agreement, either accepting it or proposing new terms, a replied agreement is sent via the web application. The agreement is signed with the data provider's private key (signature).

\item The web application submits the request with the data provider ID and the signed data provider's agreement to DDS. % content of the agreement needs to be defined

\item Once the data provider's agreement is received, DDS checks whether the data provider's account is valid, and stores the signature in the {\em directory storage}.

\item After the bi-directional agreements are both received, DDS confirms whether both parties\footnote{Note that the data consumer address and data provider address are derived from the IDs stored in the agreements, and the data consumer's signature and data provider's signature are retrieved from the {\em directory storage}. Besides, the deployment date and the validity status are set by DDS.} can enter a contract.
If so, DDS signs and sends an ESAD-TX to the {\em data directory} on the ledger.  If not, DDS returns to the
data consumer with a reason code.  The consumer can consider to rebid, or terminate.

\item The {\em data directory} creates a new ESA on the ledger. In other words, the ESA for both data provider and data consumer is established and triggered\footnote{ESA stores the data provider address, data consumer address, data certificate, data owner code (de-identified), data entry title, data description, data access path, agreement terms, data provider's agreement, data consumer's agreement, EAS deployment date and EAS validity status (set to {\em true}). Note that the data provider address, data certificate, data owner code (de-identified), data entry title, data description, data access path and data conditions are retrieved from the corresponding data entry.}.

\item After receiving the EASD-TX, the EASD-TX is stored as an activity event for {\em data activity logging}.

\item This EASD information is synchronized to the {\em directory storage} and {\em audit log storage}.
\end{enumerate}

%\begin{figure*}[ht]
%\begin{center}
%\includegraphics[width=14cm]{Images/DataXchangeWorkFlow-deployment-Alison.png}
%\end{center}
%\caption{The workflow of EAS deployment}
%\label{fig:system_workflow_deployment}
%\end{figure*}


\subsection*{ESAI \& ESAR}

\noindent
{\bf API}: {\em POST /eas/invoke/ : log an access result when an ESA is invoked} \\
\noindent
{\bf API}: {\em POST /eas/revoke/ : revoke an ESA by a user (provider or consumer)}

%\noindent Figure~\ref{fig:system_workflow_invocation} depicts the workflows of EASI and EASR.

\begin{enumerate}
\item Before an ESA deployment, the provider inserted for each data item a data registry (with data certificate and data access script) into the registry storage of the provider's data server.
\item After ESAD, the consumer is noticed that an EAS has been created. The consumer can now send a download access request for this data item via the web application.
\item The web application submits the download access request with the data consumer's signature to the provider's data server via the data access script (e.g., the provider server's REST API).
\item After receiving the request, the provider server retrieves the corresponding EAS content on the ledger to check the offer conditions, the validity status and the data consumer's signature. If the access time has expired or the validity status is {\em false}, the data download access is denied (denoted as ``validation failed''). 
\item The provider server sends a validation passed/failed result signed with the data provider's private key (signature) to DDS.
\item Once the provider server's result is received, DDS checks whether the data provider's account is registered, and then sends an ESAI-TX with the validation result to the {\em data directory} on the ledger.
\item After receiving the ESAI-TX, the EASI-TX is stored as an activity event for {\em data activity logging}.
\item On step (5), if the validation passes, the provider server sends a request to the data server (both are managed data provider service) to apply the real download link for the data consumer with an expiration time stamp. 
%The purpose of this design is to avoid real data file path exposure (on data entry) problem and download link spreading problem for security. In addition, this design also meet the timely access requirement for data expiration date.
\item The data provider thus transfers the data to the data consumer via the real download link (or access script).
\item After the data is downloaded by the data consumer, the consumer verify data authenticity via the certificate server.
\item This ESAI information is synchronized to the {\em directory storage} and {\em audit log storage}.
\item Furthermore, the data provider or data consumer can send an EASR request via the web application to DDS for revocation (disable the data access) when desired. DDS subsequently sends an ESAR-TX to the {\em data directory} on the ledger. 
%To send an EASR-TX, the form fields of data provider ID, data consumer ID and data certificate are required. Note that data provider address and data consumer address are derived from the IDs; also, the form field of validity status is set to {\em false} by DDS. An EASR-TX is signed with the data provider's private key (signature) or the data consumer's private key (signature). 
After receiving the EASR-TX, the ESAR-TX is stored as an activity event for {\em data activity logging} with
validity status set to {\em false}. 
Finally, this ESAR information is synchronized to the {\em directory storage} and {\em audit log storage}. 
Note that the data consumer cannot send the EASR request after the data has been downloaded by that consumer.
\end{enumerate}

%\begin{figure*}[ht]
%\begin{center}
%\includegraphics[width=14cm]{Images/DataXchangeWorkFlow-invocation-Alison.png}
%\end{center}
%\caption{The workflow of EAS invocation and revocation}
%\label{fig:system_workflow_invocation}
%\end{figure*}



\subsection*{DQS: Data Query Service}
\noindent
{\bf API}:{\em GET /entry/search/ : retrieve data entries with a search query}

\noindent Figure~\ref{fig:system_workflow_search} depicts the workflow of DQS.

\begin{enumerate}
\item Any registered user can log onto DDS to issue a query with desired criteria (e.g., disease name, gender,
and age) via the web application to find matching data entries.
\item DDS retrieves from its {\em directory storage} based on the query criteria.
\item DDS returns matching data entries to the querier.
\end{enumerate}


%\subsection{Non-Goals}

%In this version, we do not consider payment and negotiation to be tightly coupled. 
%Payment can be performed through e.g., debit/credit cards. For negotiation, the conditions can be initially determined and sent to DDS by data providers; the data consumers can send requests for agreement if they accept those conditions. 

%The blockchain guarantees that each replica has the same sequence of transactions and each transaction has been validated by validators in the blockchain layer.
%Second, in the blockchain layer, there are several validators wrapping validated transactions into a {\em block} and make an agreement with which block once a time during a time interval.
%(block confirm -> tx confirm) 
%According to the consensus protocol used in the blockchain layer, when a block is broadcasted or there can be different ways to confirm blocks. The confirmed blocks 



==> Architecture-Old.tex <==
\TODO{We need to replace the following section}. 
\section{Platform Architecture}
\label{sec:architecture}

This section presents \Soteria's architecture design and its key
components for supporting transactions on data items.

\subsection{Transaction Types}

A transaction is an indelible record written onto the ledger to reflect a
particular activity on a data item. For provability and auditability,
\Soteria supports five transaction types:  

\begin{enumerate}
 \item {\em User Registration} (UR).
 Each consumer and business must register an account on \Soteria.
 An UR transaction (UR-TX) consists of a user-specified ID and a public key (address). (Note that
 the term {\em user} here refers to a user of \Soteria.)
 
 %\item {\em Data Entry Creation} (DEC) and {\em Data Entry Deletion} (DED).
 %A DEC transaction (DEC-TX) consists of data provider's address, data certificate, data owner code (de-identified), data entry title, data description, data access path, access conditions (e.g., data offer price and data entry due date), data entry creation date and data-availability status (set to {\em true}). A DED transaction (DED-TX) consists of the same fields as DEC-TX, except that the data-availability status is set to {\em false}.
 
 \item {\em EAS Deployment} (EASD).
 An EAS (executable agreement script) between a user and a business describes the terms of accessing a data item (or data items). An EASD transaction (EASD-TX) includes PI owner's address, business' address, access control agreement, EAS deployment date, and EAS validity status (set to {\em true}). 
 As stated in \cite{8613656}, an EAS does not store PI but only a 
 script\footnote{Working with Stanford OVAL, EAS
 can store an EAS in natural language for auditability. \Soteria can then employ Genie \cite{Genie} to convert natural language to an executable programming script.  The public sees the smart contract in natural language but neither code nor data.} to access PI for preserving privacy. 
 
 \item {\em EAS Invocation} (EASI).
 An EASI transaction (EASI-TX) indicates that an EAS has been invoked by a business. 
 EASI-TX records which user's data item has been retrieved by which business.
 
 \item {\em EAS Revocation} (EASR).
 An EAS can be revoked by a user, and a previous EAS is 
 then deemed invalid. Since the ledger is append-only, a revocation is 
 implemented by creating a new EAS to revoke an existing one. 
% Note that the directory service keeps track of each EAS' status and makes timely revocations.
\end{enumerate}

Note that a rectification request issued by a user is executed in two consecutive transactions,
an EASR to revoke an existing consent and then an EASD to create a new consent.
The directory service first indicates that a rectification request has been received and
is pending for verification.  Once the EASR and EASD transactions have been 
executed and recorded on the ledger,
the directory service shows a successful completion status with a time stamp. 

\subsection{System Components}


\begin{figure*}[ht]
\begin{center}
\includegraphics[width=12cm]{Images/SoteriaWorkFlow-overall-Alison.png}
\end{center}
\caption{\Soteria system architecture}
\label{fig:system_architecture}
\end{figure*}

Figure~\ref{fig:system_architecture} presents the system components of \Soteria and depicts the interactions between these components. 
The three components of \Soteria are: 
\begin{itemize}
\item {\em Data directory service} (DDS): DDS stores information about all data items that are available
for exchange.
\item {\em Audit trail service} (ATS): ATS stores incurred transactions on data items for
auditing.
\item {\em Distributed ledger} (DTL): DTL is our multi-layer blockchain that satisfies \Soteria's 
requirements including privacy, throughput and latency. 
%\Soteria currently uses Ethereum \cite{} as its ledger\footnote{Though Ethereum has a latency of a few seconds, it suffices to support medical data exchange. We are continuing to investigate alternatives such as Tendermint}.
\end{itemize}

Users of \Soteria are PI owners, business, and  
auditors.  PI owners and business can elect to store and search
their respective rights on DDS.
While users can directly
access DTL by bypassing DDS, direct access cannot efficiently 
support the keeping consumers {\em informed} right required by the regulations.
DDS as a middle man cannot conceal data from the public because 
both PI owners and business can audit through consistency 
checks between DDS and DTL.

ATS caches transation records written onto DTL.
With ATS, an auditor can issue 
a request to look up all activities occurred on a specified
piece of PI.  Between DDS and DTL, 
DDS uploads a transaction onto DTL with an initial status.  
Once the transaction has been validated on DTL by e.g., a jury pool (discussed in Section~\ref{sec:protocols}),
ATS updates the status of the transaction in its local cache.  
Both DDS caching and ATS caching 
require setting two parameters:

\begin{itemize}
\item Refresh time:  How often do DDS and ATS check on DTL to update the transaction status?
\item Consistency latency:  How up-to-date is the information on DDS and ATS?  (Note that
this latency is different from DTL's consensus protocol latency.)
\end{itemize}

Between refresh time and consistency, there are tradeoffs.
The shorter the refresh time, the shorter the consistency latency between
the cache and ledger.  However,
a shorter refresh time incurs higher CPU and IO overhead.  For \Soteria,
we believe that a consistency latency of a few seconds 
for DEC may not be such a critical inconvenience.
%Analogically, Google does not crawl new Web sites in real time. 
However, for EASR (EAS Revocation) a short latency is required. 
\Soteria thus conducts different refresh cycles for different transaction types.
Given a transaction type, \Soteria further adjusts
refresh time to be reverse-proportional to the number of pending 
transactions that DDS has issued to DTL to achieve a good balance 
between latency and overhead. For instance, if very few EASI transactions have
been issued since the last refresh cycle, the refresh time can be longer.
When many EASI transactions have been issued, the refresh time can be shorter.
For timely revocation, \Soteria could withhold an EAS invocation transaction
(EASI-TX) if \Soteria has recently received an EASR-TX on that EAS and is pending
on DTL for validation.  

%The request handling is presented as follows. First, DDS sends transactions for each DEC request to the ledger, making the data entry information searchable on the directory. At the same time, the {\em directory storage} also synchronizes the data entries recorded on the ledger. Note that this ledger is used for caching the data directory information (data entries) on the ledger, improving the directory search efficiency. Second, DDS retrieves the data directory information cached from the {\em directory storage} according to DQS requests, and then returned the data entries from the search. Third, ATS retrieves the data activity log information from the {\em audit log storage} when ALR requests are received. Similar to the {\em directory storage}, the {\em audit log storage} is also used for caching the data activity log information on the ledger, improving the log retrieval efficiency. Namely, both the {\em directory storage} and {\em audit log storage} synchronize the information recorded on the ledger periodically.

\begin{comment}
\subsection{Attacks}

We discuss some attack scenarios and 
explain how \Soteria defends against them.
%We must consider all attack scenarios so that our design 
%can effectively evaluate all safety versus efficiency tradeoffs.

%Here we blur the boundary between an attack and an error. For instance, invoking an expired contract can be regarded as a non-malicious error instead of an attack. However, a case such as creating multiple entries for the same data at different prices may be an error or may be permitted depending on the policy of the system.

\leftmargini= 5.5mm
\leftmarginii= 6mm
\begin{enumerate}
 \item {Provider attacks}.
 \begin{itemize}
     \item Attack \#1. Data provider $y$ impersonates data provider $x$ to sell the data of provider $x$. 
    UR-TX validates a provider's credentials to defend this attack scenario.
    %For the more efficient validation process, they can set up access control list servers described in Section \ref{sec:auth}.
    \item Attack \#2. Data provider $x$ agrees with the data owner to provide data item $x_i$, and
    then replaces $x_i$ with $x_j$ in EAS.
    \Soteria designs DDS combined with a data certificate (DEC-TX) to provide data consumers 
    a way for validating if the data has been changed.
    \item Attack \#3. Data provider $x$ creates and sells invalid/fake data or cannot deliver the data even if EAS has been validated. Not all attack cases can be directly safeguarded by \Soteria.  Cases like these are not defendable by any protocols (analogously, one could obtain a bad product from a reputable online store).
    These attack cases can be mitigated by a data-provider reputation system.  
    %銀貨兩訖
    %\item Attack \#7. Data consumer $z$ sends the same smart contract multiple times to increase the limit of the permission of data without data provider $x$ agreeing on it.
    %reuse the smart contract after using once without data provider's agreement.
    %same as attack 3
 \end{itemize}
 \item {Consumer attacks}.
 \begin{itemize}
    \item Attack \#4. Consumer $z$ accesses the data and violates EAS terms (e.g., data expiration date). 
    An EAS that violates access terms will not be executed.  A defense 
    scheme is for DDS to periodically check 
    EAS' and issue a revocation transaction (EASR-TX) on an invalid EAS.
    \item Attack \#5. Consumer $z$ unlawfully forwards or resells a data item after purchased that data item.  This case cannot be defended even by e.g., a watermarking scheme.
    If a piece of data is leaked, at least the audit trail can narrow down the possible
    suspects.
 \end{itemize}
 \item {Validation attacks}.
  \begin{itemize}
     \item Attack \#6. A data item has multiple DEC-TXs recorded on the ledger. If
     this is not the intent of the provider, DDS can mark duplicates.
     \item Attack \#7. Fake or altered transactions were inserted to the audit trail. \Soteria as a middle man can be attacked.  However, since DTL has records of the trusted originals, 
     ATS can check with DTL to safeguard attacks of this kind.
    \item Attack \#8. The certification system is compromised. \Soteria relies on
    a trusted third-party certification system.  
  \end{itemize}
\end{enumerate}

\end{comment}

==> AuditTrail.tex <==
\section{Audit Trail}
\label{sec:audit}
Many real world workflows desire having audit trail.
For example, any supply chain can be benefited by
having digital log book using blockchain technology designed to address the evolving regulations for tracking and tracing all activities.
A hospital IRB requires to document 
activities to satisfy auditing requirements.

To make the data tamper 
proof, each log book record receives a timestamp by sending a 
cryptographic hash—or ‘fingerprint’—of the record to 
a distributed blockchain ledger. Using the hash methodology, 
all records are kept strictly confidential, while still 
providing proof that the data actually exists.
\begin{comment}
\begin{figure*}[th]
\begin{center}
\includegraphics[width=12cm]{Images/directory_service_flow.png}
\end{center}
\caption{Flowchart of directory service}
\label{fig:dsflow}
\end{figure*}

\begin{figure*}[h]
\begin{center}
\includegraphics[width=12cm]{Images/directory_service.png}
\end{center}
\caption{UML of directory service}
\label{fig:ds}
\end{figure*}


For more efficient auditing, instead directly searching data in the blockchain database, we build a directory server which is the entry of the access control list (ACL) and contracts which users signed on the blockchain. 

In Figure \ref{fig:dsflow}, data provider send a policy transaction to the blockchain. After the transaction being confirmed, every directory server will pull the latest confirmed block $B_{l}$ to their memories. 
Each block contains two kinds of transaction, policy and log, where policy transactions create or modify the authorization of data, see \ref{sec:auth}; log transactions record data access or execution results.

However, in directory service, we only need policy transactions to update the directory.
Thus, directory servers acquire policy transactions $T_{l}^P = \{t_{l}^1, t_{l}^2, t_{l}^3,...\}$ from $B_{l}$ and update the directory database according to the content of each $t_{l}^i \in T_{l}^P$.
% For example,

\subsection{Component Definition}
\begin{enumerate}
\item{\em Directory Server}
There are two features of the directory server. First, it gets the latest confirmed policy transactions from the blockchain and creates the latest data frame $d_{l}$ for them. Second, it puts $d_{l}$ into directory.
\item{\em Directory Database}
Each column of the directory records the fingerprint of the data, the data owner, proxies and proxies' access conditions. Moreover, for each proxy, the whole history of the data authorization is also written down.

% insert the JSON file with .png
\end{enumerate}
\begin{comment}
/\begin{lstlisting}

{"ColumnInd": {
  "DataOwner": "Address",
  "Fingerprint": "",
  "Signature": "",
  "Tranaction": t_0,
  "BlockNum": 1,
  "Consortium":"DataProvider",
  "Authorization": {
    "Proxy": [
      {"ProxyID": "DataConsumer_1",
      "AccessState": "Conditioned",
      "AccessConditions":[{"NumAccess":2, "Payment": 10}],
      "AuthorizationHistory":[{"Transaction": %t_1, "BlockNum":2}, 
        {"Transaction": t_2, "BlockNum":5}]},
      {"ProxyID": "DataConsumer_2",
      "AccessState": "Always",
      "AccessConditions":[],
      "AuthorizationHistory":[{"Transaction": %t_3, "BlockNum":3}]},...
      
    ]
  }
}}
\end{lstlisting}/
\end{comment}

\subsection{API Definition}
\begin{enumerate}
\item{\em Send Policy Transaction}
%There are two types of policy transaction:
%create data
%add access conditions (authorization)
\begin{itemize}
    \item POST /\{\$BLOCKCHAIN\}/\{\$ADDRESS\}/\{\$DATA\}: create a data owned by the address on the blockchain.
    \item PUT /\{\$BLOCKCHAIN\}/\{\$ADDRESS\}/\{\$DATA\}/\{\$PROXY\}: update the list of proxies for the data which is owned by the user with the address on the blockchain. This function can notify every server in the blockchain network to add authorization to the specified proxy to the data.
\end{itemize}

\item{\em Pull The Latest Block}
\begin{itemize}
\item GET /\{\$BLOCKCHAIN\}/$(\{\$LASTBLOCKNUMBER\}+1)$: retrieve the latest bock from the blockchain.
\end{itemize}

%\item{\em Update The Database}
%\begin{itemize}
%PUT /
%\end{itemize}
\item{\em Query The Directory}
\begin{itemize}
\item GET /\{\$DIRECTORY\}/\{\$CONDITION\}: retrieve the information under the condition from the directory server.
\end{itemize}
\end{enumerate}
\end{comment}

==> Authorization.tex <==
\section{Authorization}
\label{sec:auth}
% Authorization of data owner and data provider
% through blockchain
Authorization includes two parts to establish data ownership
and grant rights to access.

\subsection{ACL}

Each data has its own ACL which records which proxy has the authorization to access the data under what conditions. Conditions are written as a smart contract described in Section \ref{subsec:smart_contracts}. Once a smart contract is signed by the data owner and deployed on the blockchain successfully, the directory server will update the ACL for the data.

\subsection{Executing Smart Contracts}
\label{subsec:smart_contracts}
Though we dislike the term smart contract, we use it in this
document because of its popularity in the blockchain community.

The composition of a smart contract includes 




==> Certification.tex <==
\section{Certificate}
\label{sec:certification}

% certificate of data item and contract
Certificate is used in two scenarios. The first is to ensure the entry of each data item is available and the access path is correct to prevent data consumers from accessing the wrong data created by malicious. Second, when data providers want to sell data items, they can issue orders with conditions and prices. To protect orders from tampering, DS provide an append-only Merkle tree, like Google certificate transparency, to record orders' certificates.

\subsection{Data Certificate}
%\textcolor{red}{Discussion: DS maintains a list of trusted institutions, their public keys and their locations in its Public Key Infrastructure (PKI). Each trusted institution holds a certificate server which has the power to issue data certificates.Provider $x$ submits encrypted data $E\left(d, pk_{i}\right)$ to DS where $pk_{i}$ indicates the public key of $i_{th}$ trusted institution. Here, encryption can be done at the frontend in a cell phone or any devices even offline. Therefore, the data item would not be leaked. Then, DS searches PKI with $pk_{i}$ and sends to the location of $i_{th}$ certificate server $CS_{i}$ for asking the data certificate of $d$. $CS_{i}$ decrypts data and stores $d$ in a database. After that, it returns data certificate $C\left(d\right)$, a path $d$ stored in, and a signature signed with its private key.} 
\begin{figure*}[ht]
\begin{center}
\includegraphics[width=12cm]{Images/connection.png}
% Hand drawing is also cool. I just put the color version.
\end{center}
\caption{System connection diagram}
\label{fig:connection}
\end{figure*}
For an Institution who owns the database which is the destination that data items are stored in, there are two types of communication, vertical (black arrows in Figure \ref{fig:connection}) and horizontal (blue arrows in Figure \ref{fig:connection}), for different parties. 

A client can send requests to the destination database through the vertical gateway. However, to protect sensitive data from prowling Internet forces, DS runs a proxy server to interact with destination databases outside the Internet. 
Since the proxy server will hide databases' location if clients ask for passing their requests to databases, hackers cannot directly attack the database running the service.
Moreover, in order to save data providers' and consumers' privacy, the proxy server uses HTTPS tunnel to upload/download the encrypted data items to/from databases.


The blockchain connects institutions in the horizontal way which means each of them has the same power to maintain the distributed ledger. Also, the ledger records each data items' ownership, certificate, location, permission, and time sequence.
\begin{figure*}[ht]
\begin{center}
\includegraphics[width=12cm]{Images/data_certificate_flow.png}
% Hand drawing is also cool. I just put the color version.
\end{center}
\caption{The workflow of creating a data certificate.}
\label{fig:data_dertificate_flow}
\end{figure*}

The data certificate is created by following the steps depicted in Figure \ref{fig:data_dertificate_flow}:
\begin{enumerate}
    \item Data provider $x$ create data item $d$ for a data owner $y$ and wants $d$ to be stored into the institution $i$. First, $x$ encrypts $d$ with $i$'s public key $pk_{i}$ and gets $E\left(d, pk_{i}\right)$. After that, $x$ sends $E\left(d, pk_{i}\right)$, $y$'s signature $Sig_{O}$, $y$'s blockchain address $add_{y}$, and data certificate $C\left(d\right)$ to DS where $C\left(\cdot \right)$ is a hash function.
    \item DS verifies $x$'s permission. If $x$ has right to write the $i$'s database then sends $E\left(d, pk_{i}\right)$ and $Sig_{O}$ to $i$'s location.
    \item $i$ decrypts data, verifies $Sig_{O}$, and then store $d$ in the database. Next, it returns data certificate $C\left(d\right)'$ and its signature $Sig_{i}$ to DS.
    \item DS compares $C\left(d\right)$ and $C\left(d\right)'$. If $C\left(d\right) \neq C\left(d\right)'$, DS returns a signalto $x$. Else if two of them are equal, DS sends a data creation transaction to the blockchain. The data creation format is described as follow:
    \begin{itemize}
        \item createdata <institutionaddress> <institutionsignature> <datadescription> <owneraddress> <ownersignature> <datacertificate>
    \end{itemize}
    \item Blockchain validators validate $Sig_{i}$ and $Sig_{O}$ and then wrap them into a block if they are valid. Otherwise the data creation transaction will be dropped.
\end{enumerate}

\subsection{Order Certificate}
% proxy signature

==> Directory-Ed.tex <==
\section{Directory Service}

Similar to a browser to the Internet, the directory Service {DS} acts 
as the browser of all shared data. DS handles the transactions defined
in the previous section including 
{\em data creation}, {\em smart contract}, {\em access log}, 
and {\em revocation}. 

DS interacts with blockchain and audit trail to complete all these transactions
while storing a local copy for the metadata of these transactions to be
browsed and searched.  Note that DS does not store the data items being exchanged.
DS stores metadata and may have the access path (code) to an data item, but not the 
physical data itself.

\subsection{Data Creation}
% declare the owner and provider
Provider $x$ submits a data description $d$ and an data access path $d_{code}$
to DS.  
Since DS does not access physical data, the certification must 
be performed by the consumer with a trusted party (e.g., Google)
to obtain $C\left(d\right)$.
Once certified, 
DS uploads a $T_{dc}\left(C\left(d\right)\right)$ to the blockchain.

Once the blockchain signals creation success,
DS makes $d$ and $d_{code}$ and C$\left(d\right)$ searchable 
to the subscribers.  Internally, DS stores in its database
a tuple ($x$, $d$, $d_{code}$, C$\left(d\right)$).

{\bf
Note that $C\left(d\right)$ is created by the provider, and $d_{code}$
will be validated by a jury once a smart contract transaction has
been uploaded to the blockchain, which is discussed next.
}

\subsection{Smart Contract}

Any subscriber can search on the database to identify desired tuples.
The search is expected to be performed on data descriptions 
such as lung cancer CT or brain tumor MRI.
DS returns matching tuples to the querier.

The querier can negotiate with the provider via DS to formulate a
contract. While contract details can vary depending on the data
types and local regulations, we can assume that a typical contract 
consists of six pieces of information:
\begin{itemize}
    \item Provider (seller) $x$,
    \item Consumer (buyer) $z$,
    \item Data certificate C$\left(d\right)$,
    \item Data access path (code) $d_{code}$,
    \item Conditions, and
    \item Price.
\end{itemize}

DS then creates this contract on the blockchain.
Upon creation success (contract validated), the tuple together with
a pointer to the smart contract on the blockchain 
is stored in DS's local database. (Before the contract has been
validated, a tuple could be inserted into DS' database with
a status {\em pending for validation}.)
This tuple is made searchable only by users $x$ and $z$.

\subsection{Access Log}

Consumer $z$ after a contract has been validated on the blockchain can
execute it.  The contract is executed on the
provider's node. DS should provide a secured environment
for providers to execute the contract.  

After the contract has been executed and the consumer received the
data, the data item's certificate is validated by the consumer 
to ensure that C$\left(d\right)$ matches.

When an access transaction is issued by a consumer, DS first validates the consumer, 
and then fetches the contract from the blockchain, and then executes
the smart contract on the provider's site. The execution consists of five steps:
\begin{enumerate}
    \item Validate the consumer,
    \item Validate access conditions,
    \item Execute $d_{code}$ in the contract at the provider's site,
    \item Update conditions on the DS database, and
    \item Return $E\left(d\right)$, encrypted data, to the consumer.
\end{enumerate}

The side effects recorded on the DS database include access timestamp and access count.
The access status, successful or fail, is published onto the blockchain.

\subsection{Revocation}

==> Directory.tex <==
\section{Directory Service}

 % searchable meta data (access information)
 % each data state
 % list orders
 \begin{figure*}[th]
\begin{center}
\includegraphics[width=12cm]{Images/DirectoryServiceArchi_2_0.png}
\end{center}
\caption{The architecture of DeepLinQ directory service}
\label{fig:directory_service_archi}
\end{figure*}

The architecture of DeepLinQ directory service is depicted in Figure \ref{fig:directory_service_archi}. Clients, both data providers and data consumers, interact with the blockchain and data entities through DeepLinQ directory server. DeepLinQ directory service is based on {\em chain of trust} \footnote{\url{https://en.wikipedia.org/wiki/Chain_of_trust}} and four components are needed: {\em directory server}, {\em data directory server}, {\em data server} , and {\em entity database}. 


\begin{enumerate}
     \item {\em Directory server}. DeepLinQ directory server (DDS) associate information of domain names assigned to each of the participating entities.
     Moreover, not just like a domain name server, DDS maintains a list to record each data replica and, for each data, it records fields as below:
    \begin{enumerate}
        \item Metadata including a name, a fingerprint, and some de-identification information which are fetched from the blockchain.
        \item Smart contracts about the data deployed on the blockchain.
        \item A list of replicas and the domain they stored. In addition, each replica is assigned a flag representing the availability.
    \end{enumerate}
    \item {\em Data directory server}. A data directory server is responsible for collecting the information of a set of data servers and passing to DDS. The information carries data server IPs and a report for the availability of every data replica.
    \item {\em Data server} A data server upholds a database or a set of databases. A client can operate, reading or writing, data directly through data server if he/she is directed to the address and has enough permission; also data servers will send access log transactions to the blockchain. In addition, data servers report data  availability to data directory servers.
    \item {\em Entity database}. Data replica is stored in a entity database.
\end{enumerate}


\begin{figure*}[th]
\begin{center}
\includegraphics[width=12cm]{Images/DataCreationFlow_2_0.png}
\end{center}
\caption{The workflow of data creation}
\label{fig:data_creation_flow}
\end{figure*}
DDS provides data providers to create new data and add permission to others. Once the transactions are recorded on the blockchain, the directory service should notice all the data servers and collect responses from them. The workflow is depicted in Figure \ref{fig:data_creation_flow} and described as follow:

\begin{enumerate}
    \item Data provider $x$ sends data $E\left(d\right)$ encrypted by the public key of the destination $pk_{i}$ and the destination domain name to {\em API service} in the DDS. $E\left(\cdot
    \right)$ indicates encryption function and $d$ represents the data. Moreover, $x$ should provide a signature to prove himself.
    \item DDS finds the {\em data server} $DS_{i}$ that $x$ assigned through {\em directory service}.
    \item {\em Transaction service} delivers $E\left(d\right)$ to $DS_{i}$.
    \item $DS_{i}$ verifies $x$'s signature and decrypts $E(d)$ with $pk_{i}$ to get $d$ and save $d$ in the entity database after checking the permission of $x$. 
    \item {\em Data server} $DS_{i}$ sends data creation transaction $tc_{j}$ to the blockchain with a data fingerprint $H\left(d\right)$ and $DS_{i}$'s signature where $H\left(\cdot\right)$ indicates a hashing function. 
    \item DDS monitors the blockchain and updates the database if the new block is generated. 
    \item Once $tc_{j}$ is put in the database of {\em directory service}, DDS notifies $x$ that his/her data has been created in the whole blockchain network. Therefore, $x$ can check whether fingerprints of $d$ that $x$ holds, and contained in the $tc_{j}$ are the same.
\end{enumerate}


\begin{figure*}[th]
\begin{center}
\includegraphics[width=12cm]{Images/SmartContractTranaction.png}
\end{center}
\caption{The workflow of smart contract transaction}
\label{fig:smart_contract_flow}
\end{figure*}

Data provider $x$ can also add permission to data consumer $y$ by sending smart contract transaction. Figure \ref{fig:smart_contract_flow} shows the flow and is described as follow:

\begin{enumerate}
    \item $x$ sends a smart contract transaction to data consumer $y$ through DDS. A smart contract transaction includes a signature of the data owner, a signature of $y$ and a JSON file which clarifies $y$ accepts the contract on what condition and which files.
    \item DDS verify signatures and sends to the blockchain if they are valid.
    \item Blockchain monitors should notice the smart contract transactions and updates its access control list (ACL).
    \item DDS return the result to $x$.
\end{enumerate}



\begin{figure*}[th]
\begin{center}
\includegraphics[width=12cm]{Images/LogAccessFlow.png}
\end{center}
\caption{The workflow for data access by a data consumer.}
\label{fig:access_data_flow}
\end{figure*}

After giving data consumer $y$ the permission of data $d$, $y$ can send a request to DDS for accessing $d$.
The workflow is depicted in Figure \ref{fig:access_data_flow} and described as follow:
\begin{enumerate}
    \item Data consumer $y$ sends a request to DDS.
    \item DDS finds data server $DS_{i}$ that contains $d$.
    \item DDS sends the request to $DS_{i}$.
    \item $DS_{i}$ look up the ACL, and then access entity database for $d$ if $y$ has enough permission.
    \item In the meanwhile, $DS_{i}$ sends a log access transaction $tl_{j}$ to the blockchain.
    \item Blockchain monitors fetch the newly log access transaction from the blockchain.
    \item Once $tl_{j}$ is detected, $DS_{i}$ encrypt $d$ in $E\left(d\right)$ with $y$'s public key and returns back to the DDS.
    \item DDS delivers $E\left(d\right)$. Data provider can decrypt with his/her private key. Also, he/she can check $d$'s hash on the blockchain for verifying the correctness of $d$.
\end{enumerate}





==> Experiment-Alison.tex <==
\section{Experiments}
\label{sec:exp}

\subsection{Throughput with different input transaction rates and number of nodes}
\begin{enumerate}
\item More number of nodes can afford more transactions in a time.
\item More number of nodes can perform higher throughput.
\end{enumerate}

\begin{figure*}[ht]
\begin{center}
\includegraphics[width=10.5cm]{Images/Tendermint-InputTxRate-Throughput.png}
\end{center}
\caption{Tendermint: throughput with different input transaction rates and number of nodes}
\label{fig:tendermint_input_tx_rate_throughput}
\end{figure*}

\subsubsection{Latency with different input transaction rates and number of nodes}
\begin{enumerate}
\item Due to the network delay between nodes, latency becomes higher when more nodes are running.
\item In 1-node case, there is no network latency.
\end{enumerate}

\begin{figure*}[ht]
\begin{center}
\includegraphics[width=10.5cm]{Images/Tendermint-InputTxRate-Latency.png}
\end{center}
\caption{Tendermint: latency with different input transaction rates and number of nodes}
\label{fig:tendermint_input_tx_rate_latency}
\end{figure*}

\subsubsection{Latency and throughput with different input transaction rates and number of nodes}
\begin{enumerate}
\item The higher throughput, the higher latency.
\item The more number of nodes, the higher latency.
\end{enumerate}

\begin{figure*}[ht]
\begin{center}
\includegraphics[width=10.5cm]{Images/Tendermint-Throughput-Latency.png}
\end{center}
\caption{Tendermint: latency and throughput with different input transaction rates and number of nodes}
\label{fig:tendermint_input_tx_rate_latency_throughput}
\end{figure*}



==> Introduction-Old.tex <==
\section{Introduction}

Why do we propose a distributed ledger to facilitate data sharing?
The aim is two-fold.  First, when a data item is shared, we would like to ensure
indelible records related to that data item are hardened on the ledger.  
Second, the indelible records are transparent and decentralized, and any actions on the data item
is publicly auditable.  In this work, we focus our application on medical data, and 
name our platform MedXchange.

We design MedXchange with five functions to achieve the aim.
Some of the functions are fundamental to provide an indelible and
auditable ledger, and some are essential for making the ledge 
usable with great user experience.

DeepLinQ's five functions are:
{\em searchable directory}, 
{\em entry authentication}, 
{\em access authorization},
{\em timely revocation}, and
{\em auditability}.

\begin{enumerate}
\item {\em Data Directory}. On distributed ledgers, data can be
isolated if they cannot be made searchable.  In early days of
the Internet, Yahoo served as a directory and its usefulness started
a search engine industry.  For shared data to be discovered and searched
across distributed ledgers, a similar directory is required.
An early such directory is Hacera \cite{}.

\item {\em Data Certification}.  Every entry returned from a search
must contain a certificate ensuring that the entry has been validated.
When the data item is eventually retrieved or exchanged, the certificate
can be matched to verify the data item's authenticity. 

\item {\em Access Authorization}.  Authorization includes access control and
contracts. Access control determines the owner(s) of a data item and/or its
proxy, whereas a contract dictates the rights that the provider of
an data item grants to a consumer under a set of conditions (e.g., duration
and monetary). 

\item {\em Timely Revocation}.  When the access right to a
data item has been changed or revoked, DeepLinQ reflects
the change with low latency.

\item {\em Auditability}. All activities on all data items are
logged for open and transparent auditing.
\end{enumerate}

To support these five enumerated functions, we design DeepLinQ
data exchange platform with three components (depicted shortly)
to service users of three roles: data providers, data consumers,
and auditors.
APIs and protocols are specified to define  
the interactions between roles and 
components and between components.

\section{Preliminaries}

We define terms and depict workflow and attack cases
in this section to prepare for our detailed specifications
in Section~\ref{sec-specs}.

\subsection{Transactions}

Figure \ref{fig:system_archi} depicts the interactions between components and roles. 
Data providers send transactions to the blockchain layer
through DeepLinQ. (Though transactions can be submitted
directly to the blockchain, the {\em searchable directory} (SD) acts as 
the UI for transaction creation, submission, browsing, and search.)
Data consumers find data on SD,
and submit requests through SD to create smart contracts on
the blockchain.  Each smart contract is then validated by a pool of jurors (to
be defined).  Once a smart contract has been validated,
the contract is shown on the directory service and the data consumer of the contract
can trigger its execution to fetch data according to the contract terms (e.g.,
access duration and frequency).  All transactions are written onto
the ledger, and a copy cached by SD for quick search.

The definition of a transaction can be a general event. 
We define four transaction types in our design described below. 

\begin{enumerate}
    \item {\em Data Creation}. A data creation transaction consists of
 data owner (anonymized), data provider (data proxy), and the fingerprint of the data
 (i.e., data certificate). 
 A data provider can be the owner of the data or a proxy. 
     \item {\em Smart Contract}. A smart contract is an agreement between a data provider and a data consumer on the rights/terms to access some specified data items.
    In addition to the provider and consumer IDs, an agreement also includes
    the code to access data, data certificate, access duration, and additional 
    conditions (e.g., price) if applicable. As stated in \cite{8613656}, a contract does not
    store the data itself but the code to access the data for 
    the privacy-preserving reason. 
    \item {\em Revocation}. A smart contract can be revoked, and a previous
    validated contract is then deemed invalid.  A change to an old contract
    can be implemented as creating a new contract after revoking an existing one.
    \item {\em Access Log}. The access log transaction indicates which data 
    item (identified by its certificate ID) has been accessed 
    by which data consumer.  
\end{enumerate}

Section~\ref{subsec:smart_contracts} details how the 
code in a smart contract is constructed.
Section~\ref{sec:certification} details the certification service.
Section~\ref{sec:audit} details the auditing service built upon access log transactions.

\subsection{Workflow}

\begin{figure*}[ht]
\begin{center}
\includegraphics[width=12cm]{Images/DeepLinQWorkFlow_color.png}
% Hand drawing is also cool. I just put the color version.
\end{center}
\caption{The interactions between components and roles.}
\label{fig:system_archi}
\end{figure*}


A typical workflow depicted in Figure \ref{fig:system_archi} is as follows:
\begin{enumerate}
    \item A data provider publishes some data items via a {\em data creation} transaction.
    The transaction is created on the blockchain through the directory service.  (The
    directory service in this case provides merely user interface to the blockchain.)
    \item New transactions are monitored by the directory service, and the metadata
    of the newly created transactions after they have been validated on the blockchain
    by the jury pool (step \#5) are fetched
    to the repository of the directory service.
    \item A data consumer looks up data items on the directory service.
    The consumer selects desired data items and enters access duration (and
    an offer price if applicable).
    \item A {\em smart contract} transaction is created between the consumer
    and provider once they have reached agreement. 
    \item The {\em smart contract} is validated by a pool of jurors. 
    \item The smart contract once has been validated, can be executed by
    the data consumer according to the terms of the contract.  Whenever
    the contract is executed (and thereby data fetched), 
    an {\em access log} transaction is written onto the blockchain.
    \item An audit trail can be created to report activities on a data
    item, on a contract, on a provider, and/or on a consumer.
    \item A {\em revoke} transaction can be issued onto the blockchain to
    invalidate a previously certified smart contract.  
\end{enumerate}

This workflow and the transaction section mention several key components 
of DeepLinQ, including directory service, 
data certification, smart contracts, audit trail, and trusted exchange. 
We will detail these components in the following sections.

\subsection{Attacks}

Next, we discuss some attack scenarios and then 
explain why and how DeepLinQ defends them.
We must consider all attack scenarios so that our design 
can evaluate all safety and efficiency tradeoffs.

%Here we blur the boundary between an attack and an error. For instance, invoking an expired contract can be regarded as a non-malicious error instead of an attack. However, a case such as creating multiple entries for the same data at different prices may be an error or may be permitted depending on the policy of the system.

\begin{enumerate}
 \item {Provider attacks}.
 \begin{itemize}
     \item Attack \#1. Data provider $y$ fakes as data provider $x$ to sell the data of provider $x$. 
    %By comparing the data fingerprint of the data of $x$, data consumers can search, on the blockchain, the data creation transaction $t_x$ of the data that $x$ provided. After that, Data consumers can easily check whether the data owner field in $t_x$ is $x$ or not. For the more efficient validation process, they can set up access control list servers described in Section \ref{sec:auth}.
    \item Attack \#2. Data provider $x$ agrees to provide data item $x_i$, and 
    then replaces $x_i$ with $x_j$ in the contract. One possible case is that
    a hospital changes a patient's diagnosis to make a higher insurance claim.
    %In this case, since orders for data exchange is off-chain, any modification can not been noticed by data consumers. However, DeepLinQ designs a directory service combined with an entry certification to provide data consumers a way for validating the existence of orders based on the trust of third-parties. See Section \ref{sec:certification} 
    \item Attack \#3. Data provider $x$ creates and sells invalid/fake data 
    for self or other owners. 
    %Before sending a data creation transaction to the blockchain, $x$ and $y$ should sign the data to indicate the confirmation by both side. In addition, blockchain validators should check the signatures before receiving it. However, validators can only check the signatures, but if both the data provider and the data owner collude, signing the data, validators can not 
    \item Attack \#4. Data provider $x$ cannot deliver the smart contract even if after the contract has been validated and data consumer $y$ paid.  
    \item Attack cases that will not be directly safeguarded by DeepLinQ.  
    There are cases not defendable by any protocols
    such as a consumers sells a fake or low quality data. (One
    could obtain a bad product from any reputable Internet stores.)
    Some attack cases can only be mitigated by a provider reputation system.  
    %銀貨兩訖
 %   \item Attack \#7. Data consumer $z$ sends the same smart contract multiple times to increase the limit of the permission of data without data provider $x$ agreeing on it.
    %reuse the smart contract after using once without data provider's agreement.
    %same as attack 3
 \end{itemize}
 \item {Consumer attacks}.
 \begin{itemize}
    \item Attack \#5. Data consumer $z$ accesses the data violating the agreed contract terms (e.g., access duration and frequency). 
    %Since all access logs about the data are recorded on the blockchain, auditors can trace the log history, and smart contracts which $y$ and the data owner signed together. The audit trail is described in Section \ref{sec:audit}.
    \item Attack \#6. Consumer $z$ unlawfully forwards or resells a data item after purchased that data item.
 \end{itemize}
 \item {Validation attacks}.
  \begin{itemize}
     \item Attack \#7. A data item has multiple data creation transactions recorded on the blockchain.
      \item Attack \#8. Certification system is compromised.
      \item Attack \#9. Audit trail was inserted fake or altered transactions. 
  \end{itemize}
\end{enumerate}

\subsection{Non-Goals}

In this version, we do not consider payment to be tightly coupled.
Payment can be performed through e.g., debit/credit cards.
Additional protocol is required to validate a smart 
contract with payment.  


%The blockchain guarantees that each replica has the same sequence of transactions and each transaction has been validated by validators in the blockchain layer.


%Second, in the blockchain layer, there are several validators wrapping validated transactions into a {\em block} and make an agreement with which block once a time during a time interval.
%(block confirm -> tx confirm) 
%According to the consensus protocol used in the blockchain layer, when a block is broadcasted or there can be different ways to confirm blocks. The confirmed blocks 








 

==> Prototypes.tex <==
\section{Prototypes and Examples}



==> Revocation.tex <==
\section{Revocation}


